Multi-Agent Join

It is crucial to provide real-time performance in many applications, such as interactive and exploratory data analysis. In these settings, users often need to view subsets of query results quickly. It is challenging to deliver such results over large datasets for relational operators over multiple relations, such as join. Join algorithms usually spend a long time on scanning and attempting to join parts of relations that may not generate any result. Current solutions usually require lengthy and repeated preprocessing, which is costly and may not be possible to do in many settings. Also, they often support restricted types of joins. In this paper, we outline a novel approach for achieving efficient join processing in which a scan operator of the join learns during query execution, the portions of its relations that might satisfy the join predicate. We further improve this method using an algorithm in which both scan operators collaboratively learn an efficient join execution strategy. We also show that this approach generalizes traditional and non-learning methods for joining. Our extensive empirical studies using standard benchmarks indicate that this approach outperforms similar methods considerably.

==> sigmod-response.tex <==
We thank reviewers for their helpful comments.
Reviewer #2
O1. As explained in the introduction, since our methods treat the join condition as a black-box, they address challenges (1) and (2).
Because they learn during processing each individual query, they can handle workloads in which the distribution of queries may change over time. We will discuss how these issues are addressed by our methods throughout the revised submissions. 

O2. As noted in Section 3.1.2, current works on progressive joins, e.g., [16], show that in the absence of any specific order on R, e.g., sorted relation, sequential scan on R simulates random sampling effectively. Thus, the probability such an arrangement is very low. Like current work on progressive joins and AQP, our guarantees are for expected running times over all possible arrangements. 

O3. 1) It takes more space than a single paper to extend and evaluate our approach for queries with multiple joins as the joins in the higher levels of the query tree face a different sets of actions/costs than the ones over the base relations. We leave this as a future work. We will explain the general direction of doing so and its challenges in the revised submission. 
2) Selective joins are also challenging for other methods, such as BNLJ or [16], to handle without any index. Our empirical study shows that our methods are at least as efficient as the competing one in this setting. We will clarify the challenges and limitation of our and similar methods for this setting in the revised submission.

O4.As explained in our response to O2, sequential scan over R simulates random sampling of R. Thus, the probability of having such an arrangement is low. Also, as the competing methods, e.g., BNLJ, start from the beginning of R, they do not deliver results fast in this setting either. We discuss these worst cases in the revised submission.

O5.We will follow the reviewer's comment and compare our method with the one in [16] in the revised submission. Our goal is to process joins progressively where no indexes are available or the join condition may be complex, e.g., involve user-defined functions. Thus, some methods are not comparable to ours, e.g., [24] needs indexes. Please also read our response to D2 of Reviewer #4 about this. We will follow the reviewer's comment to empirically evaluate our method over TPCH with larger scale factors and investigate the impact of changing of the number of blocks. The skewness of input is the most influential parameter in the performance of an MAB method, which we have investigated empirically. We appreciate if the reviewer clarify what they mean by "input characteristics" and "payload size" so we include them in our revised empirical study.

Reviewer #3
O1. We will follow reviewer's comments and state the problem and algorithms formally and add examples for the algorithms in the revised submission.

O2. We will precisely state our contributions and their limitations in the introduction in the revised submission. 

O3. We will revise the title of the revised submission to reflect our contributions.

11. We meant that that work handles a restricted subset of binary joins. We will precisely describe the differences of our work with the related work in this regard in the revised submission. 

Reviewer #4
D1. We will follow the reviewer's comment and motivate the problem using concrete use-cases in AQP as well as other settings where progressive join processing is useful, e.g., [16,5].

D2. Our goal is to process joins progressively where no indexes are available or the join condition may be complex, e.g., involve user-defined functions. Some current methods, e.g., [24], require precomputed indexes. Some others, e.g., [20], may not handle binary joins with complex conditions as they use a sort-based approach. Some method in [16] does not require index and handle joins with complex conditions. However, as noted in the introduction, these methods run our of memory even over datasets of modest size, e.g., reported in [20]. To address the reviewer's comment, we compare our methods with the comparable ones in [16] empirically in the revised submission. We also compare our method with [20] for queries where sort-based approaches are applicable. We also add queries with complex conditions to our workload and discuss why some methods are not comparable to ours in the revised submission.

D3. As explained in Section 6.1.2 and 6.2.3, we use those versions of TPCH to be able to report some results for BLNJ as this method does not terminate after days over larger versions. We will compare our methods with the competing ones over larger versions of TPCH in the revised submission.

D4. We follow reviewer's comments and explain the algorithms precisely. 

D5. One may use the returned partial join results to estimate or use progressive join processing to deliver gradually more accurate estimates of aggregation functions, e.g., average [16,20,24]. We will explain how our method is used to compute aggregation functions in the revised submission.  

D6. As the reward table contains only the addresses and rewards of a subset of blocks in R, it has a relatively small memory footprint. We will describe these details precisely in the revised submission.

D7. Since both scans learn in this collaborative scan, we need some book-keeping to avoid generating duplicate results. This overhead may make it less efficient than single-scan learning over some datasets. We will explain these overheads and our justifications in detail in the revised submission.
-----
O1.We will use new queries, e.g., joins with complex functions, in our empirical studies to compare our proposed algorithms with the current ones experimentally.

D2-Some methods, however, are not comparable to ours, e.g., [24] requires indexes. 
As our learning-based approach treats the join condition as a black box, it can handle joins with complex conditions efficiently.
This is why we did not compare our methods against the ones in [16]. 
